Comparing two perfect bases

We study a class of varieties which generalize the classical orbital varieties of Joseph. We show that our generalized orbital varieties are the irreducible components of a Mirkovic-Vybornov slice to a nilpotent orbit, and can be labeled by semistandard Young tableaux. Furthermore, we prove that Mirkovic-Vilonen cycles are obtained by applying the Mirkovic-Vybornov isomorphism to generalized orbital varieties and taking a projective closure, refining Mirkovic and Vybornov's result. As a consequence, we are able to use the Lusztig datum of a Mirkovic--Vilonen cycle to determine the tableau labeling the generalized orbital variety which maps to it, and, hence, the ideal of the generalized orbital variety itself. By homogenizing we obtain equations for the cycle we started with, which is useful for computing various equivariant invariants such as equivariant multiplicity and multidegree. As an application, we show that in type $A_5$ the Mirkovic-Vilonen basis and Lusztig's dual semicanonical basis are not equal as perfect bases of the coordinate ring of the unipotent subgroup. This is significant because it shows that perfect bases are not unique. Our comparison relies heavily on the theory of measures developed in Baumann, Kamnitzer, and Knutson's MV Basis and DH Measures (2019), and we include what we need to be self-contained. Finally, we state a conjectural combinatorial "formula" for the ideal of a generalized orbital variety in terms of its tableau.

==> backmatter/colophon.tex <==
% !TeX root = ../main.tex

\begin{figure}
\caption{The generalized orbital variety whose projective closure is the MV cycle of coweight $((4,4,2,2),(2,2,2,2,2,2))$ for $SL(6)$}
\label{fig:yogi}
\hfill
% , aka \textit{the elusive Yogi}
\small
\input{figures/idealJlessbadgen.tex}
\end{figure}
% 
\begin{figure}%[ht]
    \caption{Its preprojective algebra module}
    \centering
    \definecolor{a5}{RGB}{109,61,99}
    \color{a5}
    \[
    \begin{tikzpicture}
        \begin{scope}[scale=1.4] % ,xshift=4.5cm
        \node (10) at (1,0){$2$};
        \node (30) at (3,0){$4$};
        \node (01) at (0,1){$1$};
        \node (21) at (2,1){$33$};
        \node (41) at (4,1){$5$};
        \node (12) at (1,2){$2$};
        \node (32) at (3,2){$4$};
        \node at (4.4,1){$\oplus$};
        \draw[->] (12) to node[pos=.3,left]{$\scriptstyle1$} (01);
        \draw[->] (12) to node[pos=.6,left]{$\left(\bsm1\\0\esm\right)$} (21);
        \draw[->] (32) to node[pos=.6,right]{$\left(\bsm0\\1\esm\right)$} (21);
        \draw[->] (32) to node[pos=.3,right]{$\scriptstyle1$} (41);
        \draw[->] (01) to node[pos=.6,left]{$\scriptstyle-\xi'$} (10);
        \draw[->] (21) to node[pos=.3,left]{$\left(\bsm\xi'&1\esm\right)$} (10);
        \draw[->] (21) to node[pos=.3,right]{$\left(\bsm1&1\esm\right)$} (30);
        \draw[->] (41) to node[pos=.6,right]{$\scriptstyle-1$} (30);
        % \draw (2,-.6) node{$Q_\xi$};
        \end{scope}
        \end{tikzpicture}
% \begin{tikzpicture}
% \begin{scope}[scale=1.4]
    % \node at (0,5) {$\times$};
% \end{scope}
% \end{tikzpicture}
        \begin{tikzpicture}
        \begin{scope}[scale=1.4]
        \node (10) at (1,0){$2$};
        \node (30) at (3,0){$4$};
        \node (01) at (0,1){$1$};
        \node (21) at (2,1){$33$};
        \node (41) at (4,1){$5$}; % \,\,\,\times
        \node (12) at (1,2){$2$};
        \node (32) at (3,2){$4$};
        \draw[->] (12) to node[pos=.3,left]{$\scriptstyle1$} (01);
        \draw[->] (12) to node[pos=.6,left]{$\left(\bsm1\\0\esm\right)$} (21);
        \draw[->] (32) to node[pos=.6,right]{$\left(\bsm0\\1\esm\right)$} (21);
        \draw[->] (32) to node[pos=.3,right]{$\scriptstyle1$} (41);
        \draw[->] (01) to node[pos=.6,left]{$\scriptstyle-\xi$} (10);
        \draw[->] (21) to node[pos=.3,left]{$\left(\bsm\xi&1\esm\right)$} (10);
        \draw[->] (21) to node[pos=.3,right]{$\left(\bsm1&1\esm\right)$} (30);
        \draw[->] (41) to node[pos=.6,right]{$\scriptstyle-1$} (30);
        % \draw (2,-.6) node{$Q_\xi$};
        \end{scope}
        \end{tikzpicture}
        \]
\end{figure}


% \newpage

% \thispagestyle{empty}% Reset page style to 'empty'
\begin{figure}
    \caption{Its multidegree in \(Sym (\mathfrak{sl}(6))\)} %, which differs from flag function of $M$ by a multiple of the flag function of $I(\omega_1)\oplus I(\omega_2)$
    \centering
    \tiny
    \input{figures/pierre.tex}
\end{figure}

==> backmatter/gue.tex <==
% !TeX root = ../dranowski_anne_yyyymm_phd_thesis.tex

\chapter{Grand unifying example}
% 
Let \(G = GL_m\) and fix \(\uvi \) as before. 
Recall the resulting convex order on \(\Delta_+\)
\[
\beta_1^{\uvi} \le \beta_2^{\uvi} \le \dots \le \beta_\ell^{\uvi}    
\]
with \(\beta_k^{\uvi} = w_{k-1}\alpha_k\).
% 

Our analysis relies on the maps 
\begin{equation}
    B(\lambda) \to B(\infty) \to \NN^\ell
\end{equation}
and a right inverse \(\NN^\ell \to B(\lambda)\).


==> chapters/ch5sl.tex <==
% !TeX root = ../dranowski_anne_yyyymm_phd_thesis.tex
\section{MOVE Lusztig data of MV cycles}
\label{s:ldmv}
% 
The explicit combinatorial characterization of MV cycles is given by Kamnitzer in \cite{kamnitzer2010mirkovic} for the right quotients \(G^\vee(\cO)\backslash G^\vee(\cK) \), which we denote by \(\Gr'\)
since the main ingredient in translating between right and left quotient 
% in type \(A\) 
is the transpose\footnote{On the level of the Lie algebra the transpose is the antihomomorphism that swaps $e_i$'s and $f_i$'s and fixes the Cartan subalgebra.} \(g\mapsto g'\). 
% \todo{Outside of type A}

\todo[inline]{Move me to Chapter 5}
Let \(V\) be a finite dimensional complex vector space. 
The Lusztig datum of an MV cycle is defined using the valuation
\begin{equation}
  \label{eq:val}
  \begin{split}
\val: V\otimes\cK&\to \ZZ \\
v&\mapsto k \text{ if }v\in V\otimes t^k \cO \setminus V\otimes t^{k+1} \cO\,.
  \end{split}
\end{equation}
When \(V = \CC\) we see that \(\val \) records the lowest power on an element of \(\cK\) which indeed enjoys the filtration 
\[
  \cdots \subset t^2\CC\xt \subset t\CC\xt \subset \CC\xt \subset t^{-1}\CC\xt\subset\cdots
\]
by lowest degree of indeterminate \(t\). 
% \todo[inline]{Valuation comes from filtration, \(\cdots\subset t^2\CC[t] \subset t\CC[t] \subset \CC[t] \subset t^{-1}\CC[t]\subset\cdots\). This valuation picks off lowest power. Whereas we want highest power, }
% 
Note that if \(V \) is a representation of \(G^\vee \) then \(V\otimes\cK \) is a representation of \(G^\vee(\cK)\). 

To wit, fix a highest weight vector \(v_{\omega_i^\vee}\) in the \(i\)th fundamental irreducible representation \(L(\omega_i^\vee)\) of \(G^\vee\), take \(w\in W\), and consider the map 
\begin{equation}
  \label{eq:dg}
\begin{split}
    & D_{w\omega_i}' : \Gr'\to\ZZ \\
    & \qquad G^\vee (\cO)g \mapsto \val (g\bar{w} \cdot v_{\omega_i^\vee})\,. 
\end{split}
\end{equation}
% where \(g\in G^\vee(\cK)\) acts on \(L(\omega_i^\vee) \otimes \cK\). 
Here \(\bar w\) denotes the lift of \(w\) defined in Chapter~\ref{ch:bases} and \(\bar{w} \cdot v_{\omega_i^\vee}\) is regarded as an element of \(L(\omega^\vee_i)\otimes\cK\).
% defined in Chapter~\ref{ch:bases}, Section~\ref{s:notation} 

Let \(U_w^\vee\) denote the conjugate unipotent subgroup \(\bar w U^\vee \bar{w}^{-1}\).
The functions defined by Equation~\ref{eq:dg} cut out the ``transpose'' semi-infinite cells \(\flip{S}^\mu_w = G^\vee (\cO)t^\mu U_w^\vee (\cK)\) in \(\Gr'\) as follows. 
% 
\todo[inline]{If keep, change \(\omega\)s to \(\omega^\vee\)s. If move to \(GL_m\) chapter, no need.}
\begin{lemma}[\cite{kamnitzer2010mirkovic} Lemma 2.4]
\label{lem:kamlem}
\(D_{w\omega_i}'\) is constructible and
% 
  \begin{equation}
    \label{eq:flipS}
      \flip{S}^\mu_w = \{L\in\Gr' \big| D_{w\omega_i}'(L) = \langle \mu, w\omega_i\rangle \text{ for all } i\}\,.
  \end{equation}
\end{lemma}
% 
Given a \(T^\vee\)-invariant closed subvariety \(Z\subset\Gr'\) we define the polytope \(\Phi(Z)\) to be the convex hull of coweights of \(G^\vee\) which are ``contained in'' \(Z\), \(\Phi(Z) = \Conv(\{\mu\in P\big| L_\mu\in Z\})\). 
Note that \(\Phi(Z) \subset \t_{\RR}^\ast = P\otimes\RR\). 
% 
Anderson, in \cite{anderson2003polytope}, showed
that this is the moment polytope of \(Z\) for the action of \(T^\vee\) on \(\Gr'\).
% 
\todo[inline]{If keep, change \(\omega\)s to \(\omega^\vee\)s. If move to \(GL_m\) chapter, no need.}
\begin{example}
  \label{eg:polflipS} The moment polytope of a transpose semi-infinite cell is something of a building block. 
\[
  \Phi(\overline{\flip{S}^{\mu}_w}) 
  = \{\nu\big|\langle\nu-\mu,w\cdot\omega_i\rangle\ge 0 \text{ for all } i \in I \}\,.
\]
\end{example}
% 
\todo[inline]{If keep, change \(\omega\)s to \(\omega^\vee\)s. If move to \(GL_m\) chapter, no need.}
% 
\begin{theorem}
  \label{thm:mvcmvp}
  \cite[Proposition 2.2, Theorem 3.1]{kamnitzer2010mirkovic}
Let \(M_\bullet\) be a BZ datum, and set 
\begin{equation}
  \label{eq:muw}
  \mu_w = \sum_{i\in I} M_{w\omega_i} w\alpha_i\,.
\end{equation}
Then
\begin{equation}
  \label{eq:mvc}
  Z = \overline{\{
    L\in\Gr'\big| D_{\gamma}'(L) = M_{\gamma} \text{ for all }\gamma\in\Gamma
  \}}
\end{equation}
is an MV cycle of coweight \((\mu_{w_0},\mu_{e})\).
% 
Moreover, 
\begin{equation}
  \label{eq:mvp}
  \Phi(Z) = \bigcap_{w\in W} \Phi(\overline{\flip{S}^{\mu_w}_w}) = P(M_\bullet)\,,
\end{equation}
with 
\begin{equation}
  \label{eq:Mw}
  M_{w\omega_i} = \langle\mu_w,w\omega_i\rangle\,.
\end{equation}
% 
All MV cycles (MV polytopes) arise via Equation~\ref{eq:mvc} (Equation~\ref{eq:mvp}). 
% 
\end{theorem}
% 
% \todo[inline]{Kam10 comments BZ data were introduced in BZ01 where they indexed Lusztig's canonical basis of \(U_+^\ast\). Notably, TPRs appear naturally in the case of MVPs, whereas in the case of the canonical basis their appearance is more mysterious.
% 
% Kam07 shows existence of bijections \(\cB \leftrightarrow\cP \underset{\text{And03}}{\overset{\text{implicit in}}{\leftrightarrow}} \cM\) which are isomorphisms of crystals wrt KL str on \(\cB\) and BFG str on \(\cM\).}
% 
By considering the transpose map \(gG^\vee(\cO)\mapsto G^\vee(\cO)g'\) from \(\Gr\) to \(\Gr'\) we derive the following analogous result for the semi-infinite cells \(S^\mu_w=U^\vee_w(\cK) t^\mu G^\vee(\cO) = U^\vee_w(\cK) L_\mu\) of \(\Gr\).
% 
\todo[inline]{If keep, change \(\omega\)s to \(\omega^\vee\)s. If move to \(GL_m\) chapter, no need.}
\begin{lemma}
\label{lem:easylemma}
\(G^\vee(\cO)g'\in \flip{S}^{\nu}_{ww_0}\subset \Gr'\) if and only if \(gG^\vee(\cO)\in S^\nu_w\subset \Gr\). 
% 
In particular, the order on the vertices of the MV polytope of the MV cycle to which \(gG^\vee(\cO)\) belongs is reversed, with the datum \(\nu_\bullet = (\nu_w)_{w\in W}\) for \(gG^\vee(\cO)\) defining \(\nu_\bullet' = (\nu_{ww_0})_{w\in W}\) for \(G^\vee(\cO)g'\) and 
\begin{equation}
  \label{eq:unflipS}
  % S^\nu_w = \{L\in\Gr \big| D'_{ww_0\omega_i}(L') = \langle\nu,ww_0\omega_i\rangle \text{ for all } i \in I \}\,.
  S^\nu_w = \{gG^\vee(\cO)\in\Gr \big| D'_{ww_0\omega_i}(G^\vee(\cO)g') = \langle\nu,ww_0\omega_i\rangle \text{ for all } i \in I \}\,.
\end{equation}
\end{lemma}
% 
\begin{proof}
Let \(gG^\vee(\cO) \in S^\nu_w\subset\Gr\). Then \(g = \bar wu\bar w^{-1}t^\nu\) for some \(u\in U^\vee\) and
\[
\begin{aligned}
  g'  &= t^\nu (\bar w^{-1})' u' \bar w' \\
      &= t^\nu \bar w (\bar w_0 u \bar w_0) \bar w^{-1} 
\end{aligned}    
\]
is an element of \(t^\nu U^\vee_{\bar w\bar w_0}(\cK)\).
% 
The computation
\[
\begin{aligned}
g'\bar w\bar w_0\cdot v_{\omega_i} 
      &= t^\nu \bar w\bar w_0 u\bar w_0 \bar w^{-1} \bar w\bar w_0 \cdot v_{\omega_i} \\
      &= t^\nu \bar w\bar w_0\cdot v_{\omega_i} \\
      &= t^{\langle \nu, ww_0\omega_i\rangle} v_{\omega_i}
\end{aligned}    
\] 
shows that 
\(D'_{ww_0\omega_i} (G^\vee(\cO)g') = \val(g'\bar w\bar w_0 \cdot v_{\omega_i})\) 
is equal to 
\(\langle \nu,ww_0\omega_i\rangle\) 
agreeing with Lemma~\ref{lem:kamlem}. 
\end{proof}
% 
We are thus led to define \(D_{w\omega_i} \) on \(\Gr\) by 
\begin{equation}
  \label{eq:Dw}
  D_{w\omega_i}(gG^\vee(\cO)) = D'_{ww_0\omega_i}(G^\vee(\cO)g')
\end{equation}
and to rewrite
\begin{equation}
  \label{eq:unflipdefS}
  S^\nu_w = \{L\in \Gr \big| D_{w\omega_i}(L) = \langle\nu,ww_0\omega_i\rangle \text{ for all } i\}\,.
\end{equation}
% 
Moreover, translating (or, rather, transposing) Theorem~\ref{thm:mvcmvp}, we obtain that an MV cycle \(Z'\) of coweight \((\lambda,\mu)\) in \(\Gr'\), becomes an MV cycle \(Z\) of coweight \((\mu,\lambda)\) in \(\Gr\). Pointwise, if \(L\in Z\), then \(L\in \overline{S^\lambda_{+}\cap S^\mu_{-}}\), and, in particular, 
\begin{gather*}
  D_{\omega_i}(L) = \langle\lambda,w_0\omega_i\rangle \qquad 
  D_{w_0\omega_i}(L) = \langle\mu,\omega_i\rangle\,.
\end{gather*}
% 
% TODO: More generally,\todo{Refining? Also, this closure is equal to \(\cap \overline S \ne \overline{\cap S}\)}
Overall, we have 
\begin{equation}
  \label{eq:mvctr}
  Z = 
  \overline{\{
    % L\in\Gr \big| D_{\gamma}'(L) = M_{\gamma} \text{ for all }\gamma\in\Gamma
    L\in\Gr\big| D_{w\omega_i}(L) = M_{ww_0\omega_i} 
  \}}\,. % = \langle\mu_{ww_0},ww_0\omega_i\rangle 
\end{equation}
% 
\todo[inline]{Let us emphasize (for ourselves) that the MV polytope of an MV cycle in \(\Gr_{G^\vee}\) of weight \((\mu,\lambda)\) is an MV polytope for \(G\) of weight \((\lambda,\mu)\). We will use this fact in Chapter~\ref{ch:mvs}.}
% 
Thanks to Theorem~\ref{thm:mvcmvp}, the Lusztig datum of an MV cycle \(Z\) can be defined as the Lusztig datum of its MV polytope.
% its BZ datum, or, equivalently,  
% 
In the next section, we will give an explicit formula for \(n^{\uvi}(Z)\) in terms of the constructible functions \(\{D_\gamma\}_\Gamma\)
% \todo{in type \(A\)}. 
% 
\subsection{Specializing to \texorpdfstring{\(SL_m\)}{type A}}
\label{ss:glm}
% 
Fix \(G = PGL_m\) so \(G^\vee = SL_m\). 
Recall that coweights of \(G\) are \(P^\vee = \ZZ^m/\ZZ(1,1,\dots,1)\).
% TODO: Yes, the dominant coweights index the irreducible highest weight representations of \(G^\vee\), 
% TODO: Yes, the dominant coweights can be described as partitions having at most \(m-1\) parts. 
% TODO: Yes, as coweights of \(G\) these partitions, \(P_+\), define points in \(G(\cK)\) and, hence, in \(\Gr_{G}\). 

We would like
% \todo{to review the combinatorics of} 
bases for representations of \(G\) coming from MV cycles in \(\Gr_{G^\vee}\). 
By Theorem~\ref{thm:mvcmvp}, the MV polytope of such an MV cycle is 
% an MV polytope lying in \(\t^\vee \), 
\(P(M_\bullet)\subset\t^* \) for some BZ datum \(M_\bullet\). 
% its vertices coweights of \(G^\vee\). 
% We can therefore view \(P(M_\bullet)\) as sitting in \(\t^\ast\).
% TODO: Note that the Weyl groups of G and G^v are the same 
%  

For every \(w\in W\), for every \(i\in I\), \(P(M_\bullet)\) has an edge connecting \(\mu_w\) and \(\mu_{ws_i}\) such that\todo{root not coroot ok here with ids made}
\begin{equation}
  \label{eq:siedge}
    \mu_{ws_i} - \mu_w = c(w,i) w\alpha_i\,.
\end{equation}
% 
The length of the edge \(c(w,i)\) is equal to the negative of the left-hand side of the \((w,i)\)th edge inequality (Equation~\ref{eq:eiwi})
\begin{equation}
  \label{eq:lensiedge}
    c(w,i) = - M_{w\omega_i} - M_{ws_i\omega_i} - \sum_{j\ne i} a_{ji} M_{w\omega_j}\,.
\end{equation}
In particular, \(c(w,i) \ge 0\).

Let \(\uvi\) be a reduced word and suppose \(w = w_{k-1}^{\uvi} \) and \(i = i_k\), so that 
\(ws_i = w_k^{\uvi} = w_{k-1}^{\uvi} s_{i_k}\).
Then 
\begin{equation}
  \label{eq:ildaslen}
\begin{split}
    n_k^{\uvi} :&= c(w_{k-1}^{\uvi},i_k) \\
    &= - M_{w_{k-1}^{\uvi}\omega_{i_k}} - M_{w_k^{\uvi}\omega_{i_k}} - \sum_{j\ne i_k}a_{j\,i_k} M_{w_{k-1}^{\uvi} \omega_j} \,.
\end{split}
\end{equation}
% 
Since the only nonzero nondiagonal entries of the Cartan matrix in column \(i_k\) are \(-1\)s in rows \(i_k\pm 1\), the length of the \(k\)th leg along the \(\uvi\)th path simplifies to
\begin{equation}
  \label{eq:ildsimplified}
    n_k^{\uvi} = - M_{w_{k-1}^{\uvi}\omega_{i_k}} - M_{w_k^{\uvi}\omega_{i_k}} + M_{w_{k-1}^{\uvi}\omega_{i_k - 1}} + M_{w_{k-1}^{\uvi}\omega_{i_k + 1}}\,.
\end{equation}

Now, fix \(\uvi = (1,2,\dots,m-1,\dots,1,2,1)\).
%  as in Chapter~\ref{ch:bases}, Section~\ref{ss:ssytld}. 
Recall that for this choice of reduced word
\begin{equation}\label{eq:betaA}
\begin{split}
  &\beta_1^{\uvi} = \alpha_1 , \,
  \beta_2^{\uvi} = \alpha_1 + \alpha_2 , \dots , 
  \beta_{m-1}^{\uvi} = \alpha_1+ \alpha_2+ \cdots + \alpha_{m-1} , \\
  & \, \,\vdots  \\
  &\beta_{\ell - 2}^{\uvi} = \alpha_{m-2} , \,
  \beta_{\ell-1}^{\uvi} = \alpha_{m-2} + \alpha_{m-1}, \\
  &\beta_{\ell}^{\uvi} = \alpha_{m-1}\,.
  % 
  % &(\beta_1^{\uvi})^\vee = \alpha_1^\vee , \,
  % (\beta_2^{\uvi})^\vee = \alpha_1^\vee + \alpha_2^\vee , \dots , 
  % (\beta_{m-1}^{\uvi})^\vee = \alpha_1^\vee + \alpha_2^\vee + \cdots + \alpha_{m-1}^\vee  , \\
  % & \, \,\vdots  \\
  % &(\beta_{\ell - 2}^{\uvi})^\vee = \alpha_{m-2}^\vee , \,
  % (\beta_{\ell-1}^{\uvi})^\vee = \alpha_{m-2}^\vee + \alpha_{m-1}^\vee, \\
  % &(\beta_{\ell}^{\uvi})^\vee = \alpha_{m-1}^\vee\,.
\end{split}
\end{equation} 
% 
and relabel \(\beta_k^{\uvi} \equiv \beta_{(a,b)} \) if \(\beta_k^{\uvi} = \alpha_{a,b} = \alpha_a + \cdots + \alpha_b\) for some \(1\le a \le b\le m-1\).
% \todo{All vees ok?} 
Correspondingly, the chamber weights
% \todo{Should be chamber coweights of \(G = PGL\), chamber weights of \(G^\vee = SL\); to add vees?} 
% TODO: no difference if we're working with GL!!! 
\(\Gamma\) indexing the terms occuring in Equation~\ref{eq:ildsimplified} take the simple form 
%
\begin{equation}
  \label{eq:gammaA}
\begin{aligned}
    w^{\uvi}_{k-1}\omega_{i_k + 1} &= [a\,b] & w^{\uvi}_{k-1}\omega_{i_k-1} &= [a+1\,b-1] \\
    w^{\uvi}_{k-1}\omega_{i_k} &= [a\,b-1] & w^{\uvi}_k\omega_{i_k} &= [a+1\, b]
\end{aligned}    
\end{equation}
so we can rewrite this equation and relable the \(k\)th entry of the tuple of \(\uvi\)-Lusztig data as follows. 
\[
    n_k^{\uvi} \equiv n_{(a,b)} = - M_{[a\,b-1]} - M_{[a+1\,b]} + M_{[a+1\,b-1]} + M_{[a\,b]}\,.
\]
% 
Here, as in \cite{kamnitzer2010mirkovic}, the subscript \([a\, b]\) is shorthand for the permutation of \(\omega_{b-a+1}\) that has 1s in positions \(a\) through \(b\) and zeros elsewhere. If \(b<a\) we understand \(M_{[a\,b]} \equiv 0\). 
% 

It follows that the \(\uvi\)-Lusztig datum of an MV cycle \(Z'\subset \Gr'\) is given by 
\begin{equation}
  \label{eq:Dld}
  % \begin{split}
    n(Z)_{(a,b)}  = D_{[a\, b]}'(L) - D_{[a+1\, b]}'(L) - D_{[a\, b-1]}'(L) + D_{[a+1 \, b-1]}'(L) %\\
                  % &= D_{w_0^b\omega_{b-a+1}}(L'_b) - D_{w_0^b\omega_{b-a}}(L'_b) - D_{w_0^{b-1}\omega_{b-a}}(L'_{b-1}) + D_{w_0^{b-1}\omega_{b-a-1}}(L'_{b-1})
  % \end{split}
  % n(\phantom{L})_{(a,b)} = D_{[a\, b]}'(\phantom{L}) - D_{[a+1\, b]}'(\phantom{L}) - D_{[a\, b-1]}'(\phantom{L}) + D_{[a+1 \, b-1]}'(\phantom{L})
\end{equation}
for all generic \(L\in Z'\). 
% 

We can rewrite this formula in more concrete terms.
% 
The functions defined by Equation~\ref{eq:dg} are valuations of minors. 
% If  we take G = GL_n, and 
Given 
% $\gamma \in W \omega_i$ 
a chamber weight \(\gamma\) of \(G\) % \todo{Sb \(G^\vee\)} 
and a representative \(g\in G^\vee(\cK)\), $g v_\gamma$ is the vector whose entries are the $i \times i$ minors of $g$ using $\gamma$ as the set
of columns. 
% 
This is because $L(\omega_i) = \wedge^i \CC^m$.\todo{Sb \(\PP(L(\omega_i))\)}
% 
% \todo{Joel: why? ref?}
We identify the Weyl group \(W\) of \(G\) with permutations of the alphabet \([m] =\{1,2,\dots,m\}\). 
Given \([i] = \{1,2,\dots,i\}\subset[m]\), and \(w\in W\), let \(w[i] = \{w(1),w(2),\dots,w(i)\}\). 
With this notation
% 
\begin{equation}
  \label{eq:dgminor}
  D'_{w\omega_i} (G^\vee(\cO) g ) 
  = 
  \val \det_{[i]\times w[i]}(g) 
\end{equation}
% 
is the minor of \(g\) using the first\todo{Joel: first only if upper tri?} \(i\) rows and the columns \(w[i]\). 

Given \(1\le b\le m \), let \(F_b = \Sp_{\cO}(e_1,\ldots,e_b)\) be the span of the first \(b\) basis vectors of \(\CC^m\)
and denote by \(w_0^b\) the longest element of the Weyl group of \(SL_b\).\todo{Sb PGL, as that's whose weights we're permuting?}
% 
Suppose \(g\) is also unipotent (hence, upper triangular)\todo{Joel: necc?}. Then \(D'_{[a\,b]}(G^\vee(\cO) g) = \det_{[b]\times [a\,b]}(g\big|_{F_b}) \) and we can identify \(g_b = g\big|_{F_b}\) with the \(b\times b\) upper left submatrix of \(g\), an element of \(SL_b\). 
Doing so, we can rewrite 
\(D'_{[a\,b]}(G^\vee(\cO) g) = D'_{w_0^b\omega_{b-a+1}}(SL_b(\cO) g_b)\). But this is none other than \(D_{\omega_{b-a+1}}(g_b' SL_b(\cO))\). 

Hence, if \(L = G^\vee (\cO)g\), and we denote by \(L_b'\) the point \(g'_b SL_b(\cO)\) of \(\Gr_{SL_b}\), then the formula of Equation~\ref{eq:Dld} transposes as
\begin{equation}
  \label{eq:Dldtr}
  % \begin{split}
  n(Z)_{(a,b)} = 
  D_{\omega_{b-a+1}}(L_b') - D_{\omega_{b-a}}(L_b') % \\ 
  % &\qquad 
  - D_{\omega_{b-a}}(L_{b-1}') + D_{\omega_{b-a-1}}(L_{b-1}')\,.
  % D_{w_0^b\omega_{b-a+1}}(L_b) - D_{w_0^b\omega_{b-a}}(L_b) \\ 
  % &\qquad - D_{w_0^{b-1}\omega_{b-a}}(L_{b-1}) + D_{w_0^{b-1}\omega_{b-a-1}}(L_{b-1})\,.
  % \end{split}
  % D_{[a\, b]}'(L) - D_{[a+1\, b]}'(L) - D_{[a\, b-1]}'(L) + D_{[a+1 \, b-1]}'(L)
\end{equation}

==> figures/hMo1.tex <==
% !TeX root = ../dranowski_anne_yyyymm_phd_thesis.tex
% 
% hilbert series of 17-dim'l T graded H^0(M,O(1))
\begin{figure}[ht]
    \centering
    $1+\alpha_1+\alpha_3+\alpha_1\alpha_2+\alpha_1\alpha_3+\alpha_2\alpha_3+\alpha_3\alpha_4+2\alpha_1\alpha_2\alpha_3+\alpha_1\alpha_3\alpha_4+\alpha_2\alpha_3\alpha_4+\alpha_1\alpha_2^2\alpha_3+2\alpha_1\alpha_2\alpha_3\alpha_4+\alpha_1\alpha_2^2\alpha_3\alpha_4+\alpha_1\alpha_2\alpha_3^2\alpha_4+\alpha_1\alpha_2^2\alpha_3^2\alpha_4$
    \caption{Hilbert series of 17 dimensional torus graded \(H^0(M,\cO(1))\)}
    \label{hmo1}
\end{figure}


==> figures/hMo2.tex <==
% !TeX root = ../dranowski_anne_yyyymm_phd_thesis.tex
% 
% hilbert series of 110-dim'l T graded H^0(M,O(2))
\begin{figure}[ht]
    \centering
    $1+\alpha_1+\alpha_3+\alpha_1^2+\alpha_1\alpha_2+\alpha_1\alpha_3+\alpha_2\alpha_3+\alpha_3^2+\alpha_3\alpha_4+\alpha_1^2\alpha_2+\alpha_1^2\alpha_3+2\alpha_1\alpha_2\alpha_3+\alpha_1\alpha_3^2+\alpha_2\alpha_3^2+\alpha_1\alpha_3\alpha_4+\alpha_2\alpha_3\alpha_4+\alpha_3^2\alpha_4+\alpha_1^2\alpha_2^2+2\alpha_1^2\alpha_2\alpha_3+\alpha_1\alpha_2^2\alpha_3+\alpha_1^2\alpha_3^2+2\alpha_1\alpha_2\alpha_3^2+\alpha_2^2\alpha_3^2+\alpha_1^2\alpha_3\alpha_4+2\alpha_1\alpha_2\alpha_3\alpha_4+\alpha_1\alpha_3^2\alpha_4+\alpha_2\alpha_3^2\alpha_4+\alpha_3^2\alpha_4^2+2\alpha_1^2\alpha_2^2\alpha_3+2\alpha_1^2\alpha_2\alpha_3^2+2\alpha_1\alpha_2^2\alpha_3^2+2\alpha_1^2\alpha_2\alpha_3\alpha_4+\alpha_1\alpha_2^2\alpha_3\alpha_4+\alpha_1^2\alpha_3^2\alpha_4+3\alpha_1\alpha_2\alpha_3^2\alpha_4+\alpha_2^2\alpha_3^2\alpha_4+\alpha_1\alpha_3^2\alpha_4^2+\alpha_2\alpha_3^2\alpha_4^2+\alpha_1^2\alpha_2^3\alpha_3+3\alpha_1^2\alpha_2^2\alpha_3^2+\alpha_1\alpha_2^3\alpha_3^2+2\alpha_1^2\alpha_2^2\alpha_3\alpha_4+3\alpha_1^2\alpha_2\alpha_3^2\alpha_4+3\alpha_1\alpha_2^2\alpha_3^2\alpha_4+\alpha_1\alpha_2\alpha_3^3\alpha_4+\alpha_1^2\alpha_3^2\alpha_4^2+2\alpha_1\alpha_2\alpha_3^2\alpha_4^2+\alpha_2^2\alpha_3^2\alpha_4^2+2\alpha_1^2\alpha_2^3\alpha_3^2+\alpha_1^2\alpha_2^3\alpha_3\alpha_4+4\alpha_1^2\alpha_2^2\alpha_3^2\alpha_4+\alpha_1\alpha_2^3\alpha_3^2\alpha_4+\alpha_1^2\alpha_2\alpha_3^3\alpha_4+\alpha_1\alpha_2^2\alpha_3^3\alpha_4+2\alpha_1^2\alpha_2\alpha_3^2\alpha_4^2+2\alpha_1\alpha_2^2\alpha_3^2\alpha_4^2+\alpha_1\alpha_2\alpha_3^3\alpha_4^2+\alpha_1^2\alpha_2^4\alpha_3^2+3\alpha_1^2\alpha_2^3\alpha_3^2\alpha_4+2\alpha_1^2\alpha_2^2\alpha_3^3\alpha_4+\alpha_1\alpha_2^3\alpha_3^3\alpha_4+3\alpha_1^2\alpha_2^2\alpha_3^2\alpha_4^2+\alpha_1\alpha_2^3\alpha_3^2\alpha_4^2+\alpha_1^2\alpha_2\alpha_3^3\alpha_4^2+\alpha_1\alpha_2^2\alpha_3^3\alpha_4^2+\alpha_1^2\alpha_2^4\alpha_3^2\alpha_4+2\alpha_1^2\alpha_2^3\alpha_3^3\alpha_4+2\alpha_1^2\alpha_2^3\alpha_3^2\alpha_4^2+2\alpha_1^2\alpha_2^2\alpha_3^3\alpha_4^2+\alpha_1\alpha_2^3\alpha_3^3\alpha_4^2+\alpha_1^2\alpha_2^4\alpha_3^3\alpha_4+\alpha_1^2\alpha_2^4\alpha_3^2\alpha_4^2+2\alpha_1^2\alpha_2^3\alpha_3^3\alpha_4^2+\alpha_1^2\alpha_2^2\alpha_3^4\alpha_4^2+\alpha_1^2\alpha_2^4\alpha_3^3\alpha_4^2+\alpha_1^2\alpha_2^3\alpha_3^4\alpha_4^2+\alpha_1^2\alpha_2^4\alpha_3^4\alpha_4^2$
    \caption{Hilbert series of 110 dimensional torus graded \(H^0(M,\cO(2))\)}
    \label{hmo2}
\end{figure}

==> figures/idealJbadgen.tex <==
% !TeX root = ../dranowski_anne_yyyymm_phd_thesis.tex
% 
% the degree 6 generator of yogi
${a}_{9}^{2} {b}_{2}^{2} {b}_{11}^{2}-{a}_{6}^{2} {b}_{5}^{2} {b}_{11}^{2}-2 {a}_{5} {a}_{9} {b}_{2} {b}_{6} {b}_{11}^{2}+{a}_{5}^{2} {b}_{6}^{2} {b}_{11}^{2}+2 {a}_{2} {a}_{6} {b}_{5} {b}_{9} {b}_{11}^{2}-{a}_{2}^{2} {b}_{9}^{2} {b}_{11}^{2}-2 {a}_{8} {a}_{9} {b}_{2}^{2} {b}_{11} {b}_{12}+2 {a}_{6}^{2} {b}_{4} {b}_{5} {b}_{11} {b}_{12}+2 {a}_{5} {a}_{8} {b}_{2} {b}_{6} {b}_{11} {b}_{12}+2 {a}_{4} {a}_{9} {b}_{2} {b}_{6} {b}_{11} {b}_{12}-2 {a}_{4} {a}_{5} {b}_{6}^{2} {b}_{11} {b}_{12}-2 {a}_{2} {a}_{6} {b}_{5} {b}_{8} {b}_{11} {b}_{12}-2 {a}_{2} {a}_{6} {b}_{4} {b}_{9} {b}_{11} {b}_{12}+2 {a}_{2}^{2} {b}_{8} {b}_{9} {b}_{11} {b}_{12}+{a}_{8}^{2} {b}_{2}^{2} {b}_{12}^{2}-{a}_{6}^{2} {b}_{4}^{2} {b}_{12}^{2}-2 {a}_{4} {a}_{8} {b}_{2} {b}_{6} {b}_{12}^{2}+{a}_{4}^{2} {b}_{6}^{2} {b}_{12}^{2}+2 {a}_{2} {a}_{6} {b}_{4} {b}_{8} {b}_{12}^{2}-{a}_{2}^{2} {b}_{8}^{2} {b}_{12}^{2}+2 {a}_{9}^{2} {b}_{2} {b}_{3} {b}_{11} {b}_{13}-2 {a}_{6} {a}_{7} {b}_{5}^{2} {b}_{11} {b}_{13}-2 {a}_{5} {a}_{9} {b}_{3} {b}_{6} {b}_{11} {b}_{13}-2 {a}_{5} {a}_{9} {b}_{2} {b}_{7} {b}_{11} {b}_{13}+2 {a}_{5}^{2} {b}_{6} {b}_{7} {b}_{11} {b}_{13}+4 {a}_{2} {a}_{7} {b}_{5} {b}_{9} {b}_{11} {b}_{13}-2 {a}_{2} {a}_{3} {b}_{9}^{2} {b}_{11} {b}_{13}-2 {a}_{8} {a}_{9} {b}_{2} {b}_{3} {b}_{12} {b}_{13}+2 {a}_{6} {a}_{7} {b}_{4} {b}_{5} {b}_{12} {b}_{13}+4 {a}_{5} {a}_{8} {b}_{3} {b}_{6} {b}_{12} {b}_{13}-2 {a}_{4} {a}_{9} {b}_{3} {b}_{6} {b}_{12} {b}_{13}-2 {a}_{5} {a}_{8} {b}_{2} {b}_{7} {b}_{12} {b}_{13}+4 {a}_{4} {a}_{9} {b}_{2} {b}_{7} {b}_{12} {b}_{13}-2 {a}_{4} {a}_{5} {b}_{6} {b}_{7} {b}_{12} {b}_{13}-2 {a}_{2} {a}_{7} {b}_{5} {b}_{8} {b}_{12} {b}_{13}-2 {a}_{2} {a}_{7} {b}_{4} {b}_{9} {b}_{12} {b}_{13}+2 {a}_{2} {a}_{3} {b}_{8} {b}_{9} {b}_{12} {b}_{13}+{a}_{9}^{2} {b}_{3}^{2} {b}_{13}^{2}-{a}_{7}^{2} {b}_{5}^{2} {b}_{13}^{2}-2 {a}_{5} {a}_{9} {b}_{3} {b}_{7} {b}_{13}^{2}+{a}_{5}^{2} {b}_{7}^{2} {b}_{13}^{2}+2 {a}_{3} {a}_{7} {b}_{5} {b}_{9} {b}_{13}^{2}-{a}_{3}^{2} {b}_{9}^{2} {b}_{13}^{2}-2 {a}_{8} {a}_{9} {b}_{2} {b}_{3} {b}_{11} {b}_{14}+2 {a}_{6} {a}_{7} {b}_{4} {b}_{5} {b}_{11} {b}_{14}-2 {a}_{5} {a}_{8} {b}_{3} {b}_{6} {b}_{11} {b}_{14}+4 {a}_{4} {a}_{9} {b}_{3} {b}_{6} {b}_{11} {b}_{14}+4 {a}_{5} {a}_{8} {b}_{2} {b}_{7} {b}_{11} {b}_{14}-2 {a}_{4} {a}_{9} {b}_{2} {b}_{7} {b}_{11} {b}_{14}-2 {a}_{4} {a}_{5} {b}_{6} {b}_{7} {b}_{11} {b}_{14}-2 {a}_{2} {a}_{7} {b}_{5} {b}_{8} {b}_{11} {b}_{14}-2 {a}_{2} {a}_{7} {b}_{4} {b}_{9} {b}_{11} {b}_{14}+2 {a}_{2} {a}_{3} {b}_{8} {b}_{9} {b}_{11} {b}_{14}+2 {a}_{8}^{2} {b}_{2} {b}_{3} {b}_{12} {b}_{14}-2 {a}_{6} {a}_{7} {b}_{4}^{2} {b}_{12} {b}_{14}-2 {a}_{4} {a}_{8} {b}_{3} {b}_{6} {b}_{12} {b}_{14}-2 {a}_{4} {a}_{8} {b}_{2} {b}_{7} {b}_{12} {b}_{14}+2 {a}_{4}^{2} {b}_{6} {b}_{7} {b}_{12} {b}_{14}+4 {a}_{2} {a}_{7} {b}_{4} {b}_{8} {b}_{12} {b}_{14}-2 {a}_{2} {a}_{3} {b}_{8}^{2} {b}_{12} {b}_{14}-2 {a}_{8} {a}_{9} {b}_{3}^{2} {b}_{13} {b}_{14}+2 {a}_{7}^{2} {b}_{4} {b}_{5} {b}_{13} {b}_{14}+2 {a}_{5} {a}_{8} {b}_{3} {b}_{7} {b}_{13} {b}_{14}+2 {a}_{4} {a}_{9} {b}_{3} {b}_{7} {b}_{13} {b}_{14}-2 {a}_{4} {a}_{5} {b}_{7}^{2} {b}_{13} {b}_{14}-2 {a}_{3} {a}_{7} {b}_{5} {b}_{8} {b}_{13} {b}_{14}-2 {a}_{3} {a}_{7} {b}_{4} {b}_{9} {b}_{13} {b}_{14}+2 {a}_{3}^{2} {b}_{8} {b}_{9} {b}_{13} {b}_{14}+{a}_{8}^{2} {b}_{3}^{2} {b}_{14}^{2}-{a}_{7}^{2} {b}_{4}^{2} {b}_{14}^{2}-2 {a}_{4} {a}_{8} {b}_{3} {b}_{7} {b}_{14}^{2}+{a}_{4}^{2} {b}_{7}^{2} {b}_{14}^{2}+2 {a}_{3} {a}_{7} {b}_{4} {b}_{8} {b}_{14}^{2}-{a}_{3}^{2} {b}_{8}^{2} {b}_{14}^{2}$


==> figures/idealJlessbadgen.tex <==
% !TeX root = ../dranowski_anne_yyyymm_phd_thesis.tex
% 
% degree < 6 generators of yogi
$
\bgroup\begin{matrix}
{b}_{15},{b}_{10},{b}_{1},{a}_{15},{a}_{10},{a}_{1}\\
{a}_{14} {b}_{11}-{a}_{13} {b}_{12}-{a}_{12} {b}_{13}+{a}_{11} {b}_{14}\\
{a}_{12} {b}_{6}+{a}_{14} {b}_{7}+{a}_{6} {b}_{12}+{a}_{7} {b}_{14}\\
{a}_{11} {b}_{6}+{a}_{13} {b}_{7}+{a}_{6} {b}_{11}+{a}_{7} {b}_{13}\\
{a}_{12} {b}_{2}+{a}_{14} {b}_{3}+{a}_{2} {b}_{12}+{a}_{3} {b}_{14}\\
{a}_{11} {b}_{2}+{a}_{13} {b}_{3}+{a}_{2} {b}_{11}+{a}_{3} {b}_{13}\\
{a}_{7} {b}_{2}-{a}_{6} {b}_{3}-{a}_{3} {b}_{6}+{a}_{2} {b}_{7}\\
{a}_{12} {a}_{13}-{a}_{11} {a}_{14}\\
{a}_{6} {a}_{12}+{a}_{7} {a}_{14}\\
{a}_{2} {a}_{12}+{a}_{3} {a}_{14}\\
{a}_{6} {a}_{11}+{a}_{7} {a}_{13}\\
{a}_{2} {a}_{11}+{a}_{3} {a}_{13}\\
{a}_{3} {a}_{6}-{a}_{2} {a}_{7}\\
{a}_{5} {a}_{6} {b}_{11}-{a}_{2} {a}_{9} {b}_{11}-{a}_{4} {a}_{6} {b}_{12}+{a}_{2} {a}_{8} {b}_{12}+{a}_{5} {a}_{7} {b}_{13}-{a}_{3} {a}_{9} {b}_{13}-{a}_{4} {a}_{7} {b}_{14}+{a}_{3} {a}_{8} {b}_{14}\\
{a}_{9} {a}_{13} {b}_{3}-{a}_{8} {a}_{14} {b}_{3}+{a}_{7} {a}_{14} {b}_{4}-{a}_{7} {a}_{13} {b}_{5}-{a}_{5} {a}_{13} {b}_{7}+{a}_{4} {a}_{14} {b}_{7}-{a}_{3} {a}_{14} {b}_{8}+{a}_{3} {a}_{13} {b}_{9}-{a}_{5} {a}_{7} {b}_{13}+{a}_{3} {a}_{9} {b}_{13}+{a}_{4} {a}_{7} {b}_{14}-{a}_{3} {a}_{8} {b}_{14}\\
{a}_{9} {a}_{11} {b}_{3}-{a}_{8} {a}_{12} {b}_{3}+{a}_{7} {a}_{12} {b}_{4}-{a}_{7} {a}_{11} {b}_{5}-{a}_{5} {a}_{11} {b}_{7}+{a}_{4} {a}_{12} {b}_{7}-{a}_{3} {a}_{12} {b}_{8}+{a}_{3} {a}_{11} {b}_{9}-{a}_{5} {a}_{7} {b}_{11}+{a}_{3} {a}_{9} {b}_{11}+{a}_{4} {a}_{7} {b}_{12}-{a}_{3} {a}_{8} {b}_{12}\\
{a}_{9} {a}_{13} {b}_{2}-{a}_{8} {a}_{14} {b}_{2}+{a}_{6} {a}_{14} {b}_{4}-{a}_{6} {a}_{13} {b}_{5}-{a}_{5} {a}_{13} {b}_{6}+{a}_{4} {a}_{14} {b}_{6}-{a}_{2} {a}_{14} {b}_{8}+{a}_{2} {a}_{13} {b}_{9}-{a}_{5} {a}_{6} {b}_{13}+{a}_{2} {a}_{9} {b}_{13}+{a}_{4} {a}_{6} {b}_{14}-{a}_{2} {a}_{8} {b}_{14}\\
{a}_{5} {a}_{7} {a}_{13}-{a}_{3} {a}_{9} {a}_{13}-{a}_{4} {a}_{7} {a}_{14}+{a}_{3} {a}_{8} {a}_{14}\\
{a}_{5} {a}_{6} {a}_{13}-{a}_{2} {a}_{9} {a}_{13}-{a}_{4} {a}_{6} {a}_{14}+{a}_{2} {a}_{8} {a}_{14}\\
{a}_{5} {a}_{7} {a}_{11}-{a}_{3} {a}_{9} {a}_{11}-{a}_{4} {a}_{7} {a}_{12}+{a}_{3} {a}_{8} {a}_{12}
\end{matrix}\egroup$
${a}_{9}^{2} {b}_{2}^{2} {b}_{11}^{2}-{a}_{6}^{2} {b}_{5}^{2} {b}_{11}^{2}-2 {a}_{5} {a}_{9} {b}_{2} {b}_{6} {b}_{11}^{2}+{a}_{5}^{2} {b}_{6}^{2} {b}_{11}^{2}+2 {a}_{2} {a}_{6} {b}_{5} {b}_{9} {b}_{11}^{2}-{a}_{2}^{2} {b}_{9}^{2} {b}_{11}^{2}-2 {a}_{8} {a}_{9} {b}_{2}^{2} {b}_{11} {b}_{12}+2 {a}_{6}^{2} {b}_{4} {b}_{5} {b}_{11} {b}_{12}+2 {a}_{5} {a}_{8} {b}_{2} {b}_{6} {b}_{11} {b}_{12}+2 {a}_{4} {a}_{9} {b}_{2} {b}_{6} {b}_{11} {b}_{12}-2 {a}_{4} {a}_{5} {b}_{6}^{2} {b}_{11} {b}_{12}-2 {a}_{2} {a}_{6} {b}_{5} {b}_{8} {b}_{11} {b}_{12}-2 {a}_{2} {a}_{6} {b}_{4} {b}_{9} {b}_{11} {b}_{12}+2 {a}_{2}^{2} {b}_{8} {b}_{9} {b}_{11} {b}_{12}+{a}_{8}^{2} {b}_{2}^{2} {b}_{12}^{2}-{a}_{6}^{2} {b}_{4}^{2} {b}_{12}^{2}-2 {a}_{4} {a}_{8} {b}_{2} {b}_{6} {b}_{12}^{2}+{a}_{4}^{2} {b}_{6}^{2} {b}_{12}^{2}+2 {a}_{2} {a}_{6} {b}_{4} {b}_{8} {b}_{12}^{2}-{a}_{2}^{2} {b}_{8}^{2} {b}_{12}^{2}+2 {a}_{9}^{2} {b}_{2} {b}_{3} {b}_{11} {b}_{13}-2 {a}_{6} {a}_{7} {b}_{5}^{2} {b}_{11} {b}_{13}-2 {a}_{5} {a}_{9} {b}_{3} {b}_{6} {b}_{11} {b}_{13}-2 {a}_{5} {a}_{9} {b}_{2} {b}_{7} {b}_{11} {b}_{13}+2 {a}_{5}^{2} {b}_{6} {b}_{7} {b}_{11} {b}_{13}+4 {a}_{2} {a}_{7} {b}_{5} {b}_{9} {b}_{11} {b}_{13}-2 {a}_{2} {a}_{3} {b}_{9}^{2} {b}_{11} {b}_{13}-2 {a}_{8} {a}_{9} {b}_{2} {b}_{3} {b}_{12} {b}_{13}+2 {a}_{6} {a}_{7} {b}_{4} {b}_{5} {b}_{12} {b}_{13}+4 {a}_{5} {a}_{8} {b}_{3} {b}_{6} {b}_{12} {b}_{13}-2 {a}_{4} {a}_{9} {b}_{3} {b}_{6} {b}_{12} {b}_{13}-2 {a}_{5} {a}_{8} {b}_{2} {b}_{7} {b}_{12} {b}_{13}+4 {a}_{4} {a}_{9} {b}_{2} {b}_{7} {b}_{12} {b}_{13}-2 {a}_{4} {a}_{5} {b}_{6} {b}_{7} {b}_{12} {b}_{13}-2 {a}_{2} {a}_{7} {b}_{5} {b}_{8} {b}_{12} {b}_{13}-2 {a}_{2} {a}_{7} {b}_{4} {b}_{9} {b}_{12} {b}_{13}+2 {a}_{2} {a}_{3} {b}_{8} {b}_{9} {b}_{12} {b}_{13}+{a}_{9}^{2} {b}_{3}^{2} {b}_{13}^{2}-{a}_{7}^{2} {b}_{5}^{2} {b}_{13}^{2}-2 {a}_{5} {a}_{9} {b}_{3} {b}_{7} {b}_{13}^{2}+{a}_{5}^{2} {b}_{7}^{2} {b}_{13}^{2}+2 {a}_{3} {a}_{7} {b}_{5} {b}_{9} {b}_{13}^{2}-{a}_{3}^{2} {b}_{9}^{2} {b}_{13}^{2}-2 {a}_{8} {a}_{9} {b}_{2} {b}_{3} {b}_{11} {b}_{14}+2 {a}_{6} {a}_{7} {b}_{4} {b}_{5} {b}_{11} {b}_{14}-2 {a}_{5} {a}_{8} {b}_{3} {b}_{6} {b}_{11} {b}_{14}+4 {a}_{4} {a}_{9} {b}_{3} {b}_{6} {b}_{11} {b}_{14}+4 {a}_{5} {a}_{8} {b}_{2} {b}_{7} {b}_{11} {b}_{14}-2 {a}_{4} {a}_{9} {b}_{2} {b}_{7} {b}_{11} {b}_{14}-2 {a}_{4} {a}_{5} {b}_{6} {b}_{7} {b}_{11} {b}_{14}-2 {a}_{2} {a}_{7} {b}_{5} {b}_{8} {b}_{11} {b}_{14}-2 {a}_{2} {a}_{7} {b}_{4} {b}_{9} {b}_{11} {b}_{14}+2 {a}_{2} {a}_{3} {b}_{8} {b}_{9} {b}_{11} {b}_{14}+2 {a}_{8}^{2} {b}_{2} {b}_{3} {b}_{12} {b}_{14}-2 {a}_{6} {a}_{7} {b}_{4}^{2} {b}_{12} {b}_{14}-2 {a}_{4} {a}_{8} {b}_{3} {b}_{6} {b}_{12} {b}_{14}-2 {a}_{4} {a}_{8} {b}_{2} {b}_{7} {b}_{12} {b}_{14}+2 {a}_{4}^{2} {b}_{6} {b}_{7} {b}_{12} {b}_{14}+4 {a}_{2} {a}_{7} {b}_{4} {b}_{8} {b}_{12} {b}_{14}-2 {a}_{2} {a}_{3} {b}_{8}^{2} {b}_{12} {b}_{14}-2 {a}_{8} {a}_{9} {b}_{3}^{2} {b}_{13} {b}_{14}+2 {a}_{7}^{2} {b}_{4} {b}_{5} {b}_{13} {b}_{14}+2 {a}_{5} {a}_{8} {b}_{3} {b}_{7} {b}_{13} {b}_{14}+2 {a}_{4} {a}_{9} {b}_{3} {b}_{7} {b}_{13} {b}_{14}-2 {a}_{4} {a}_{5} {b}_{7}^{2} {b}_{13} {b}_{14}-2 {a}_{3} {a}_{7} {b}_{5} {b}_{8} {b}_{13} {b}_{14}-2 {a}_{3} {a}_{7} {b}_{4} {b}_{9} {b}_{13} {b}_{14}+2 {a}_{3}^{2} {b}_{8} {b}_{9} {b}_{13} {b}_{14}+{a}_{8}^{2} {b}_{3}^{2} {b}_{14}^{2}-{a}_{7}^{2} {b}_{4}^{2} {b}_{14}^{2}-2 {a}_{4} {a}_{8} {b}_{3} {b}_{7} {b}_{14}^{2}+{a}_{4}^{2} {b}_{7}^{2} {b}_{14}^{2}+2 {a}_{3} {a}_{7} {b}_{4} {b}_{8} {b}_{14}^{2}-{a}_{3}^{2} {b}_{8}^{2} {b}_{14}^{2}$
% \end{figure}
% \hspace*{-\textwidth}
% \end{minipage}%


==> frontmatter/abstract.tex <==
% !TeX root = ../main.tex

\doublespacing
\chapter{Abstract}

- Font size must be a minimum of 10 points.

- Lines of text must be double-spaced.

- Abstract must not exceed 350 words for a doctoral thesis.

- Left margin should be at least 1 1/4 (32 mm); the remaining three margins should be at least 3/4 (20 mm) to the main text.

- The student’s thesis title, degree and year of convocation, full name, name of graduate department, and name of university must appear on the top of the abstract’s first page. This information is not included in the 350-/150-word count.

- Symbols, as well as foreign words and phrases, must be clearly and accurately displayed.

- Graphs, charts, tables, and illustrations are not included. 
